Boundary-Aware Dense Feature Indicator for Single-Stage 3D Object Detection from Point Clouds

3D object detection based on point clouds has become more and more popular. Some methods propose localizing 3D objects directly from raw point clouds to avoid information loss. However, these methods come with complex structures and significant computational overhead, limiting its broader application in real-time scenarios. Some methods choose to transform the point cloud data into compact tensors first and leverage off-the-shelf 2D detectors to propose 3D objects, which is much faster and achieves state-of-the-art results. However, because of the inconsistency between 2D and 3D data, we argue that the performance of compact tensor-based 3D detectors is restricted if we use 2D detectors without corresponding modification. Specifically, the distribution of point clouds is uneven, with most points gather on the boundary of objects, while detectors for 2D data always extract features evenly. Motivated by this observation, we propose DENse Feature Indicator (DENFI), a universal module that helps 3D detectors focus on the densest region of the point clouds in a boundary-aware manner. Moreover, DENFI is lightweight and guarantees real-time speed when applied to 3D object detectors. Experiments on KITTI dataset show that DENFI improves the performance of the baseline single-stage detector remarkably, which achieves new state-of-the-art performance among previous 3D detectors, including both two-stage and multi-sensor fusion methods, in terms of mAP with a 34FPS detection speed.

==> sec_analysis.tex <==
\section{Motivation}
We first briefly review PointPillars encoder (Sec. \ref{motivation-review}), which serves as the baseline discussed in this work. We then analyze the underlying reasons for introducing the context-sensitive encoder (Sec. \ref{motivation-analysis}).


\begin{figure}
    \centering
    \begin{minipage}[t]{0.95\linewidth}
        \includegraphics[width=1.0\linewidth]{img/dist}
    \end{minipage}%
    \caption{The ratio of valid points distribution of PointPillars and CTRNet pillar. Valid points mean that it contains valid information and not being zero paddings. We show the accumulated ratio of the pillar with the increasing ratio of valid points. }
    \label{fig:dist}
\end{figure}

\begin{table}[!tbh]
\begin{center}
\scalebox{0.8}{
\begin{tabular}{|c|c|c|c|c|}
\hline
Method & Moderate  & Inference Time (ms) \\ \hline
Baseline(1 FC) & 76.62  & 4.0\\ 
PointNet(4 FC) & 76.78  &11.5\\ 

\hline
\end{tabular}
}
\end{center}
\caption{3D object detection AP on KITTI val split. We compare inference time and AP among different local feature learner.}
\label{analysis:deeper}

\end{table}


\subsection{Review of PointPillars Encoder}
\label{motivation-review}
Suppose that point cloud $\mathcal{X}=\{x_1, x_2, ..., x_n\}$ with $x_i \in \mathbb{R}^{4}$, where $\mathbb{R}^{4}$ denotes coordinates $x, y, z$ and reflectance $r$. PointPillars encoder takes $\mathcal{X}$ as input and process it to a sparse pseudo-image. It first creates a set of pillars $\mathcal{P}$ with $|\mathcal{P}|=B$ by discretizing the point cloud into an evenly spaced grid in the x-y plane. It limits the maximum number of non-empty pillars as $P$ and the maximum number of points in each pillar as $N$ to exploit the sparsity of the point cloud, which generates a tensor of size $(P, N, 4)$ (4 denotes x, y, z, and intensity). Also, if the number of points in a pillar is less than $k$, then zero paddings are applied, which makes the tensor fixed in size and friendly to hardware optimization.

It then augment points in each $\mathcal{P}$ with $x_c, y_c, z_c, x_p$ and $y_p$, where the $c$ subscript represents distance to the centroid of all points in the $\mathcal{P}$ and the $p$ subscript represents the offset from the x, y center of $\mathcal{P}$.  After the augmentation, it define a set function $f: \mathcal{X}_{\mathcal{P}}^a \rightarrow \mathcal{P}_f$ that maps augmented points $\mathcal{X}^a_{\mathcal{P}} = \{x_1^a, x_2^a, ..., x_B^a\}$ with $x_i^a \in \mathbb{R}^9$ in $\mathcal{P}$ to a pillar feature vector $\mathcal{P}_f \in \mathbb{R}^C$:


$$f(\mathcal{X}^a_{\mathcal{P}})=\operatorname{MAX}_{i=1, \ldots, n}\left\{h\left(x_{i}\right)\right\}$$

Where $h$ is a single fully connected layer followed by batch normalization and ReLU, note that those $\mathcal{X}_{\mathcal{P}}^a$ are processed concurrently, and weights and gradients are shared.


% to the non-empty pillar
% to points used for learning in each pillar

Finally, it scatters the sparse pseudo-image of size $(P, C)$ back to the original pillar position to create a dense pseudo-image of size $(H, W, C)$, where H and W denote the height and width of the image.

%with a simplified version of PointNet $\varphi$
\subsection{Analysis}
\label{motivation-analysis}

% as its encoder allows the detector to be end-to-end learned with only 2D convolution layers, which is supportive of hardware acceleration. However, 
% PointPillars achieves an impressive trade-off between speed and performance. However
Though simple, PointPillars does not consider different context knowledge for each pillar to sample informative points, which not only degrades both speed and performance of the detector but also limits its ability to take full advantage of modern point set learning networks.

 For clarification, we first investigate the distribution of the ratio of valid points to points used for feature learning in each pillar in PointPillars, as shown in Fig. \ref{fig:dist}. We observe that 1) most of the pillars are not full of valid points but nearly full with zero paddings. Only one in a thousand has a ratio of valid points bigger than $75\%$, which is highly unbalanced. 2) scattered distribution brings many outlying pillars, which degrades the learning of the encoder since it treats each pillar equally. 3) PointPillars sample nearly all points in the pillar for feature learning. Consequently, noisy points that are detrimental for localizing objects are thus included. These three phenomena make the optimization of the model more difficult, which reduces the performance of the model. Moreover, too many sampling points also increase the amount of computation for learning corresponding features. Finally, they make it hard for PointPillars to explore modern deep encoder. Direct replacement of the point set learning network with existing powerful architectures, such as the deeper version of PointNet, does not bring decent improvements, but bring a significant computational overhead, as illustrated in Table. \ref{analysis:deeper}. 
 
 According to the above analysis, we propose to design a module that explicitly samples points that are beneficial for objects localization and eliminates noisy points to solve above-mentioned problems simultaneously. The advantage of the proposed context-sensitive point sampling for increasing the ratio of valid points can be seen from Fig. \ref{fig:dist}.


\begin{figure}
    \centering
    \begin{minipage}[t]{1.0\linewidth}
        \includegraphics[width=1.0\linewidth]{img/CTnet}
    \end{minipage}%
    \caption{Network structure of PointCSE and PointPillars. We illustrate how   a single non-empty pillar is processed by different encoders. While PointPillars simply take all points in each pillar for feature learning, our PointCSE sample points with dense semantic and localization and eliminate noisy points. In practice, pillars are consumed concurrently by the encoder for efficient utilization of GPU.}
    \label{fig:ctnet}
\end{figure}



%According to the above analysis, 

%we summarize two basic guidelines to explore an efficient encoders: (1) The number of valid points in each pillar should be nearly equal. (2) Effective points should be explicitly sampled. 

%    \item \textbf{Lack of Global Context Aggregation}: Modeling global context has been proven to be important for the success of point cloud learning\cite{,,,t}, especially for fine-grained tasks such as segmentation. However, PointPillar only operates on the local level and fails to consider this knowledge. We thus explore the use of global context for 3D object detection.


%
%\begin{table}[!tbh]
%\centering
%\scalebox{0.68}{
%\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
%\hline
%Method           &    Extra Time (ms) &$AP_M$ &$AP_E$ & $AP_H$\\ \hline
%%      PointPillars           & 16 &87.95       &  89.80    &   86.44   \\ \hline
%PointPillars \& 3x3 DeConv & 33 &88.31 & 90.87 & 86.82 \\
%PointPillars \& DS-DeConv      &  9 & 88.28 &  90.00     &  86.88 \\ \hline
%PointPillars \& DENFI (3x3 DeConv)       & 33 &  \textbf{88.64}       &  92.68    & \textbf{87.28}   \\ 
%PointPillars \& DENFI (DS-DeConv)     &  9 &   88.45       &   \textbf{93.87}    &   87.27 \\  \hline
%\end{tabular}}
%\caption{Comparison of DS-DeConv and DeConv in terms of performance and speed. We present extra time imposed by different DeConv design.}
%\label{ablation:ds-dconv}
%\end{table}

